Natural Boundary Conditions for Smoothing in Geometry Processing

In geometry processing, smoothness energies are commonly used to model scattered data interpolation, dense data denoising, and regularization during shape optimization. The squared Laplacian energy is a popular choice of energy and has a corresponding standard implementation: squaring the discrete Laplacian matrix. For compact domains, when values along the boundary are not known in advance, this construction bakes in low-order boundary conditions. This causes the geometric shape of the boundary to strongly bias the solution. For many applications, this is undesirable. Instead, we propose using the squared Frobenious norm of the Hessian as a smoothness energy. Unlike the squared Laplacian energy, this energy's natural boundary conditions (those that best minimize the energy) correspond to meaningful high-order boundary conditions. These boundary conditions model free boundaries where the shape of the boundary should not bias the solution locally. Our analysis begins in the smooth setting and concludes with discretizations using finite-differences on 2D grids or mixed finite elements for triangle meshes. We demonstrate the core behavior of the squared Hessian as a smoothness energy for various tasks.

==> acks.tex <==
NSERC grant
CRC
Ladislav Kavan
Denis Zorin
Ladislav's undergrad student
Yu Wang

Paul's Bellairs workshop

Dagstuhl Computational Interaction workshop


==> bbw.tex <==
% !TEX root = hessian.tex

\subsection{Bounded biharmonic weights}
\label{sec:bbw}

\begin{figure}
 \centering
  \includegraphics[width=\linewidth]{images/cactus/cactus.pdf}
  \caption{
  \alec{I like where this is going. It really does beg for a comparison to the
  deformation without the holes. Small note: I wonder if you raise the arm on
  the left if you could pack this figure a bit more w.r.t whitespace. We should
  probably also show one of the handle's weight functions with isolines in an
  inset for each. Oh! Could you make each hole look like a cowboy gunshot hole?}
  Deformation of a cactus using bounded biharmonic weights and bounded Hessian weights.
  Because there are many holes in the interior, classical bounded biharmonic weights leads to more distortion than bounded Hessian weights.
   \label{fig:bbwimg}}
\end{figure}

Bounded biharmonic weights, as described in \cite{bbwcitation} also profit from using the Hessian energy.
On the boundaries of the deforming shape it is reasonable to use zero Neumann boundary conditions, since they represent actual physical barriers.
However if there are holes in the interior that are not part of the actual shape, but possibly a result of bad input data, the boundaries of these holes should be ignored as much as possible.
This is where it makes sense to use the Hessian natural boundary conditions instead of zero Neumann boundary conditions.
To do this, the only change needed is \oded{TODO: Describe actual change from classical BBW}.

 An example is shown in Figure \ref{fig:bbwimg}: the shape of the holes in the interior is better preserved using the Hessian with natural boundary conditions than with classical bounded biharmonic weights.


==> ccsxml.tex <==
%%
%% CONCEPTS (ref. http://dl.acm.org/ccs.cfm)
%%
%\begin{CCSXML}
%<ccs2012>
%<concept>
%<concept_id>10002950.10003714.10003715.10003750</concept_id>
%<concept_desc>Mathematics of computing~Discretization</concept_desc>
%<concept_significance>500</concept_significance>
%</concept>
%<concept>
%<concept_id>10002950.10003714.10003715.10003724</concept_id>
%<concept_desc>Mathematics of computing~Numerical differentiation</concept_desc>
%<concept_significance>300</concept_significance>
%</concept>
%<concept>
%<concept_id>10010147.10010371.10010396.10010398</concept_id>
%<concept_desc>Computing methodologies~Mesh geometry models</concept_desc>
%<concept_significance>300</concept_significance>
%</concept>
%<concept>
%<concept_id>10010405.10010432.10010442</concept_id>
%<concept_desc>Applied computing~Mathematics and statistics</concept_desc>
%<concept_significance>300</concept_significance>
%</concept>
%</ccs2012>
%\end{CCSXML}
%
%\ccsdesc[500]{Mathematics of computing~Discretization}
%\ccsdesc[300]{Mathematics of computing~Numerical differentiation}
%\ccsdesc[300]{Computing methodologies~Mesh geometry models}
%\ccsdesc[300]{Applied computing~Mathematics and statistics}
%
% The next three commands are required, and insert the user-generated keywords, 
% The CCS concepts list, and the rights management text.
% Please make sure there is a blank line between each of these three commands.
%
%\keywordlist
%
%\conceptlist
%
%\printcopyright
%


==> cover.tex <==
% Why is it so hard to get a new page...
\newpage
\clearpage
\pagebreak
\newpage
\clearpage
\pagebreak
\thispagestyle{empty}
\onecolumn

\large{\textbf{List of changes since SIGGRAPH 2017 submission}}

Dear reviewers,
\vspace*{1cm}

We have significantly improved our paper based on the thorough reviews we
received during the SIGGRAPH 2017 review cycle (\texttt{paper\_0532}).
%
The most noticeable change is that we have refocused the paper around our
contribution to modeling smoothness for geometry processing problems.
%
We show results on flat 2D domains with irregular boundaries and --- new to this
submission --- 3D surfaces represented as triangles meshes.
%
Thanks to the previous reviews, we have clarified the exposition of our
contribution and more clearly delineated our work from previous methods.
%
The paper has been largely rewritten and \emph{all} figures are new or improved.

We made the following high-level changes:

\begin{enumerate}
\item Rewrote and revised the introduction and related work, removing the
feature chart table contrasting image processing and geometry processing. We
clarified that methods in image processing (e.g., for inpainting) consider
irregular domains, but with low-order boundary conditions.
\item Added new figures demonstrating data smoothing and interpolation using
the squared Hessian energy on surfaces with open boundaries (Figs.
\ref{fig:hemisphere}, \ref{fig:chimp}, \ref{fig:beetle}, and \ref{fig:phone}).
\item Introduced a novel geometric flow based on minimizing $L_1$ norm of the
Hessian (see \reffig{l1-bunny}).
\item To create such results, utilized a novel discretization of the squared
Hessian energy on triangle meshes via mixed finite element method.
(see \refsec{mFEM}).
\item Since our original submission, Wang et al.~\shortcite{Wang2015} have
released an erratum clarifying that the discrete energy in their paper differs
from the one used in their code \cite{WangError17}. We show that \emph{both}
energies have precedents in other previous works:
\begin{itemize}
\item the discrete energy used by Bergou et
al.~\shortcite{Bergou2006} does not converge to its intended continuous solution
or minimizers of other related energies for problems on flat domains.
\item a second order smoothness energy built using previous
discrete exterior calculus operators \cite{fisher2007dtv} does not preserve null
    space dimensionality.
\end{itemize}
\end{enumerate}


Our submission includes specific changes to address previous reviews:

\begin{enumerate}
  \item Included an alternative discretization to finite differences
  (\refsec{mFEM}).
  \item Generalized our results to 3D surfaces (\refsec{3d}).
  \item Removed the ``sailboat story'' and ``knowledge boundaries'' term (see
  revised \reffig{fisherman}).
  \item Improved language when addressing previous works.
  \item Clarified use of term ``irregular.''
  \item Added citations to \cite{GNRBfFRS2016,Chen:2015:BDH}.
  \item Clarified how natural boundary conditions ``emerge'' in 1D case
  (\refsec{warm-up}).
  \item Moved Green's identities into main text.
  \item Explained inner product ($\X:\Y$) notation in main text.
  \item Improved shape deformation examples (Figs.~\ref{fig:lsd-dec-vs-ours}
        and \ref{fig:cactus}).
  \item Directly compared eigen modes of various energies/boundary conditions
  (\reffig{modal-analysis}).
  \item Clarified how energies are equivalent when fully constrained
  (\refsec{equivalence} and \reffig{mn}).
  \item Added passage discussing equal computational complexity of our method
  and previous works.
  \item Corrected typos and grammar issues noticed by reviewers.
\end{enumerate}
\vspace*{1cm}


Thank you for your time. Sincerely,

Authors




==> data-smoothing.tex <==
% !TEX root = hessian.tex

\subsection{Dense Data smoothing}
\label{sec:data-smoothing}

Variational data smoothing optimizes for a function $u$ that
simultaneously satisfies a \emph{smoothness} term and \emph{data} energy term
(commonly a least-squares energy with respect to the noisy input function $f$):
%
\begin{equation}
\label{equ:data-smoothing}
%
 u = \argmin_{u} \int\limits_Ω \left( u(x) - f(x) \right)^2 \dA -
 w_\text{smooth} E_\text{smooth}(u),
\end{equation}
%
where $w_\text{smooth}$ parameterizes the amount of smoothness versus data
faithfulness. 
%
There are many options for the smoothness energy $E_\text{smooth}$.

%
%\begin{figure}
% \centering
%  \includegraphics[width=0.5\textwidth]{images/cheese_rigs/cheese_both.pdf}
%  \caption{The cheeseman jumps in the top row, trips in the
%  bottom, powered by Hessian weight functions.
%  \label{fig:cheeseman}}
% %\end{center}
%\end{figure}
%

In \reffig{omegasmoothing}, we can see that  $E_\text{smooth} ← E_{∆²}$
with natural boundary conditions will not smooth noisy data along the boundary
$∂Ω$ (left).

In geometry processing, a common remedy is to use $E_\text{smooth} ← E_{∆²}$
\emph{subject to} zero Neumann boundary conditions (see, e.g.,
\cite{Weinkauf2010}).
%
However, this makes a strong assumption that the underlying data should vary
only tangentially along $∂Ω$: high boundary influence (center).
%
If the intended influence of the boundary is not know \emph{a priori}, then
$E_\text{smooth} ← E_{\H²}$ (with natural boundary conditions) correctly models
$∂Ω$ as a ``knowledge boundary'' (right).


\begin{figure}
 \centering
  \includegraphics[width=0.5\textwidth]{images/nokia/nokia.pdf}
  \caption{Noisy heat data on the model of an old phone. The model is a very noisy surface reconstruction. The Laplacian with zero Neumann produces a solution where the isolines are very sensitive to small holes in the surface (as indicated by arrows), while the Hessian has no such issues.
  \label{fig:phone}}
 %\end{center}
\end{figure}

\begin{figure}
 \centering
  \includegraphics[width=0.5\textwidth]{images/lion/lion.pdf}
  \caption{Noisy data on a faulty scan of a lion's head. The smoothing generated by the Laplacian with zero Neumann boundary conditions is heavily influenced by the position and scale of the holes in the face, while the Hessian ignores the holes (as indicated by arrows).
  \label{fig:lion}}
 %\end{center}
\end{figure}

\oded{todo} A descriptive text about the phone figure, Figure \ref{fig:phone}. More descriptive text about the lion figure, Figure \ref{fig:lion}.




\quad

\quad

\quad


The hallmarks of smoothing with $E_\text{smooth} ← E_{∆²}$ \emph{subject to}
zero Neumann boundary conditions are isolines meeting the boundary at a
right angle for contour plots (see \reffig{pacman}) and ``lips'' at the
boundary for height-field surfaces (see \reffig{greece}).
%
In contrast, solutions smoothed with $E_\text{smooth} ← E_{\H²}$ \emph{ignore}
the boundary if the data $f$ \emph{also} ignores the boundary.

Many previous methods in image processing have considered other norms of the
Hessian for smoothness terms over image rectangles (see, e.g.,
\cite{lefkimmiatis2013hessian}).
%
In \reffig{squarel1}, we confirmed that our discretizations can be used for 
the $L_1$-norm of the Hessian with natural
boundary conditions $E_{|\H|}$
to the $L_1$-norm of the Laplacian $E_{|∆|}$ with explicitly enforced zero
Neumann boundary conditions.
%
In the spirit of self-containment, we include a standard derivation for
optimizing these energies as a quadratic program in \refapp{qp}.
%
\reffig{cathedral} extends these energies to arbitrarily bounded domains.
%
We observe that for each $L¹$ energy the behavior of its natural boundary
conditions emerges not just at the boundary of $Ω$ but also at the
places where energy concentrates: along \emph{creases} between roughly
piecewise-linear patches for $E_{|\H|}$ and at isolated high-energy spikes for
$E_{|∆|}$.


==> energies.tex <==
\section{The Laplacian and Hessian energies}

The behavior (and indeed even the shear existence) of solutions to partial differential equations is intimately linked to prescribing correct and meaningful boundary conditions. E.g., the famous Dirichlet energy, whose minimization leads to harmonic functions, requires the use of either Dirichlet or Neumann boundary conditions \cite[Chapter 11]{Jost2007}. Unfortunately, though, not both conditions can be imposed at the same locations --- as much as this would be desirable in certain applications, such as character deformation.\\

Solutions to the Laplace equation \(\Delta u = 0\) in the domain \(\Omega\) with Dirichlet boundary \(g\) on \(\partial \Omega\) conditions can be found by solving the corresponding variational problem \cite[Chapter 8.3]{Jost2007}:
\begin{equation}\label{eq:dirichletenergy}
	\argmin_{u \in H^2(\Omega), \; u|_{\partial\Omega}=g} \int_\Omega \left| \nabla u \right|^2 \dx
\end{equation}

This method is used for character animation in \cite{Joshi2007}. However using the Laplace equation as a basis for finding smooth solution to boundary values has a drawback: we can only impose Dirichlet or Neumann boundary conditions, but not both. Yet many applications need to prescribe Dirichlet boundary conditions as well as having some control over Neumann boundary conditions. In character animation for example, having no control over Neumann boundary conditions leads to spikes and discontinuities at rigging handles, as discussed in \cite{Jacobson2011}. \\

To solve this problem, we can instead look at solutions for the biharmonic equation:
\begin{equation}
	\Delta^2 u = 0
\end{equation}
The biharmonic equation is popular in elasticity, and thus there is a lot of literature on the topic. There one can find proofs for the existence of smooth solutions for simultaneous Dirichlet and Neumann boundary conditions (for example in \cite{Bacuta2003}). Its variational formulation is dependent on what kind of boundary conditions are used. We review a weak formulation for the biharmonic equation. \\

Let \(u \in C^\infty(\Omega) \) be our trial function and \(v \in C^\infty(\Omega) \) our test function. We do the normal integral to find a weak formulation:
\begin{equation}\begin{split}\label{eq:normalharmoniccalc}
	\int_\Omega v \Delta^2 u \dx &= -\int_\Omega \nabla v \cdot \nabla\Delta u \dx + \int_{\partial\Omega} v \nabla \Delta u \cdot \dA \\
	&= \int_\Omega \Delta u \Delta v \dx + \int_{\partial\Omega} \left(v \nabla \Delta u - \Delta u \nabla v \right) \cdot \dA
\end{split}\end{equation}
This was done using Green's identity. Using just differential operators and coordinate notation (with Einstein sumation), this becomes: 
\begin{equation}\begin{split}\label{eq:partialharmonic}
	\int_\Omega v & \partial_i\partial_i\partial_j\partial_j u \dx = -\int_\Omega \partial_i v \partial_i\partial_j\partial_j u \dx + \int_{\partial\Omega} v \partial_i\partial_j\partial_j u \;\dA_i \\
	&= \int_\Omega \partial_i\partial_i v \partial_j\partial_j u \dx + \int_{\partial\Omega} \left( v \partial_i\partial_j\partial_j u - \partial_i v \partial_j\partial_j u \right) \;\dA_i
\end{split}\end{equation}

Let us now review a few variational problems based on this weak formulation. Consider minimizing the following energy, the \emph{Laplacian} energy over all functions \(u \in C^\infty(\Omega)\):
\begin{equation}\begin{split}\label{eq:laplacianenergy}
	E_L(u) = \int_\Omega \left(\Delta u \right)^2 \dx
\end{split}\end{equation}

If we take an arbitrary variation \(v \in C^\infty(\Omega) \) and minimize the variational functional \(E_L(u + \varepsilon v)\) at \(\varepsilon=0\), we get (ref.\ (\ref{eq:normalharmoniccalc})):
\begin{equation}\begin{split}\label{eq:naturalbdryconds}
	0 &= \int_\Omega \Delta u \Delta v \dx + \int_{\partial\Omega} \left(\Delta u \nabla v - v \nabla \Delta u\right) \cdot \dA
\end{split}\end{equation}

This means minimizers of the biharmonic energy solve the biharmonic equation if and only if they fulfill its \emph{natural boundary conditions}:
\begin{equation}\label{eq:laplnaturalboundaryconditions}
	\textrm{for } v \in C^\infty, \quad \int_{\partial\Omega} \left(\Delta u \nabla v - v \nabla \Delta u\right) \cdot \dA = 0
\end{equation}
These do not look like anything that is commonly in use. For example, all harmonic functions fulfill them by default, which leads to a large variety of solutions. The biharmonic energy operator will be an operator with a very large null space that is hard to solve. \\

However, the minimization of biharmonic energy is used in computer graphics, for example in \cite{Jacobson2011}. The authors don't focus on the natural boundary conditions in these works. From the way mixed finite elements are used to discretize the biharmonic energy it becomes clear that zero Neumann conditions are imposed, and in addition the value of the function at certain points is fixed (Dirichlet). This means, when they minimize, they don't take an arbitrary variation \(v \in C^\infty(\Omega) \): their \(v\) is vero at the boundary with zero normal gradient. This means (\ref{eq:naturalbdryconds}) becomes:
\begin{equation}\begin{split}\label{eq:zeroneumannbdryconds}
	0 &= \int_\Omega \Delta u \Delta v \dx
\end{split}\end{equation}
which legitimizes the discretization of the biharmonic energy to solve the biharmonic equation. \\

However, there is no reason to do the integration by parts the way it was done in (\ref{eq:normalharmoniccalc}). Inspired by the notation in (\ref{eq:partialharmonic}) we can try to just switch the orders in which we do integration by parts (since derivatives in the different coordinates commute):
\begin{equation}\begin{split}\label{eq:partialhessian}
	\int_\Omega v & \partial_i\partial_i\partial_j\partial_j u \dx = -\int_\Omega \partial_i v \partial_i\partial_j\partial_j u \dx + \int_{\partial\Omega} v \partial_i\partial_j\partial_j u \;\dA_i \\
	&= \int_\Omega \partial_i\partial_j v \partial_i\partial_j u \dx + \int_{\partial\Omega} v \partial_i\partial_j\partial_j u \;\dA_i - \int_{\partial\Omega} \partial_i v \partial_i\partial_j u \;\dA_j
\end{split}\end{equation}

We can rewrite this in more traditional vector calculus notation. We introduce the expression \(H_u\) for the Hessian of the function and \(A : B = \tr(A^T B) \) for the trace inner product of two matrices.
\begin{equation}\begin{split}\label{eq:normalhessiancalc}
	\int_\Omega v \Delta^2 u \dx &= \int_\Omega H_u : H_v \dx + \int_{\partial\Omega} \left(v \left( \nabla \Delta u \right)^T - \nabla v^T H_u \right) \;\dA
\end{split}\end{equation}

This motivates the definition of a new energy, the \emph{Hessian} energy:
\begin{equation}\begin{split}\label{eq:hessianenergy}
	E_H(u) = \int_\Omega || H_u ||_F^2 \dx
\end{split}\end{equation}
where \(|| \cdot ||_h\) is the Frobenius matrix norm.

If we take an arbitrary variation \(v \in C^\infty(\Omega) \) and minimize the variational functional \(E_H(u + \varepsilon v)\) at \(\varepsilon=0\), we get (ref.\ (\ref{eq:normalhessiancalc})):
\begin{equation}\begin{split}\label{eq:naturalbdrycondshess}
	0 &= \int_\Omega H_u : H_v \dx + \int_{\partial\Omega} \left(v \left( \nabla \Delta u \right)^T - \nabla v^T H_u \right) \;\dA
\end{split}\end{equation}

This means that the natural boundary conditions for the Hessian energy are:
\begin{equation}\label{eq:hessnaturalboundaryconditions}
	\textrm{for } v \in C^\infty, \quad \int_{\partial\Omega} \left(v \left( \nabla \Delta u \right)^T - \nabla v^T H_u \right) \;\dA = 0
\end{equation}

This is equivalent to the following (ref.\ Section \ref{sec:hessianbdryderivation} in the Appendix):
\begin{equation}\begin{split}\label{eq:nicehessianbdryconds}
	\mathbf{n}^T H_u \mathbf{n} &= 0 \quad \textrm{ on } \partial\Omega \\
	\nabla \left( \mathbf{t}^T H_u \mathbf{n} \right) \cdot \mathbf{t} + \nabla \Delta u \cdot \mathbf{n} &= 0 \quad \textrm{ on } \partial\Omega
\end{split}\end{equation}
where \(\mathbf{n}\) is the normal vector on the (oriented) boundary of the domain and \(\mathbf{t}\) is the tangent vector. The second boundary condition becomes replaced by Dirichlet boundary conditions, if they are imposed.

These boundary conditions also appear in the physical interpretation of the elastic deformations of a thin plate. The variational formulation for that problem uses an energy, which is a combination of the Hessian and the Laplacian energies, as mentioned in \cite[p.\ 250]{couranthilbert}. This thin-plate energy has also been used in image processing in works such as \cite{terzopoulos}.

The first of these natural boundary conditions is now very intuitive: it corresponds to \emph{linear extrapolation}, i.e.\ the function should continue as linearly as possible across the boundary. For many applications where the boundary is not an actual physical boundary this is much more intuitive than the zero Neumann boundary conditions that are widely used. \\

Another intuitive understanding of the difference between the Laplacian and the Hessian energy can be seen by looking at the kernels of the functions. The pure Laplacian energy has all harmonic functions in its kernel: this means the matrix has a large null space and will not transform harmonic input at all. The Laplacian energy with zero Neumann boundary conditions only measures zero on constant functions. The Hessian energy however measures zero energy for constant and linear functions - this means that minimizing the Hessian energy will result in a solution that is \emph{as linear as possible} --- this is desirable for many applications, which will be presented in the following section.


==> point-constraints.tex <==
\newtheorem{lemma}{Lemma}
%
\section{Point Constraints for Biharmonic Problems}
%
\label{app:point-constraints-proof}

Let $\Omega \subset \RR^2$ be an open, bounded set with smooth boundary, and let $x_0 \in \Omega$ be some point in $\Omega$. 
%
%Consider the solution $u$ of
%\begin{align*}
%\Delta^2 u (x) &= 0 \ , \ x\in \Omega\setminus \{x_0\} \ , \\
%u(x) &=f(x) \ , \ \partial_n u(x) = g(x) \ , x\in \partial \Omega \ ,\\
%u(x_0) &= \nabla u(x_0) = 0 \ .
%\end{align*}
%
\paragraph*{Problem statement} Let $\varepsilon >0$ be small enough such that the $\varepsilon$-ball $B_\varepsilon(x_0)$ around $x_0$ is entirely contained in $\Omega$. Consider the solution $u_\varepsilon$ of 
\begin{align*}
\Delta^2 u_\varepsilon (x) &= 0 \ , \ x\in \Omega\setminus B_\varepsilon(x_0) \ , \\
u_\varepsilon(x) &=f(x) \ , \ \partial_n u_\varepsilon(x) = g(x) \ , x\in \partial \Omega \ ,\\
u_\varepsilon(x) &= \partial_n u_\varepsilon(x) = 0 \  , x\in \partial B_\varepsilon(x_0) \ . 
\end{align*}
We are interested in the limit
\[
\lim_{\varepsilon\to 0 }u_\varepsilon \ .
\]
%Is it true that $\lim_{\varepsilon\to 0 }u_\varepsilon(x) = u(x)$ for all $x\in \Omega\setminus \{x_0\}$? If so, in which topology? 
In particular, we would like to know if there exists a function $u_0 \in H^2(\Omega)$ with $u_0(x_0)= \nabla u_0(x_0) =0$ and $\Delta^2 u_0 = 0$ on $\Omega \setminus \{x_0\}$ such that 
\[
\lim_{\varepsilon\to 0 }u_\varepsilon= u_0 \quad \text{on} \  \Omega \setminus B_\delta (x_0) \quad \text{for all $\varepsilon < \delta$} \ . 
\] 
If this is so, in which topology can we expect convergence? 


\paragraph*{The general handle problem} Notice that it suffices to solve the above problem in order to solve the general ``handle problem'' that we are interested in. Indeed, suppose that we had a solution for the above problem. Let $w:\RR^2 \to \RR$ be some linear function.  Define boundary conditions $f:= -w$ and $g := -\partial_n w$ on $\partial \Omega$. Let $u_\varepsilon$ be as a above for these BCs and define 
\[
v_\varepsilon := u_\varepsilon + w \quad \text {and} \quad v_0:= u_0+w \ .
\]
Then $v_\varepsilon$ satisfies the boundary value problem
\begin{align*}
\Delta^2 v_\varepsilon (x) &= 0 \ , \ x\in \Omega\setminus B_\varepsilon(x_0) \ , \\
v_\varepsilon(x) &= \partial_n v_\varepsilon(x) = 0 \ , x\in \partial \Omega \ ,\\
v_\varepsilon(x) &= w(x) \ , \ \partial_n v_\varepsilon(x) =  \partial_n w(x) \  , x\in \partial B_\varepsilon(x_0) \ ,
\end{align*}
and we would have convergence 
\[
\lim_{\varepsilon\to 0 }v_\varepsilon= v_0 \quad \text{on} \  \Omega \setminus B_\delta (x_0) \quad \text{for all $\varepsilon < \delta$} \ ,
\] 
where $v_0 \in H^2(\Omega)$ satisfies $v_0(x_0)= w(x_0)$, $\nabla v_0(x_0) =\nabla w(x_0)$, and $\Delta^2 v_0 = 0$ on $\Omega \setminus \{x_0\}$.

\paragraph*{Filling the hole} A first idea might be to trivially extend $u_\varepsilon$ to all of $\Omega$ by setting $u_\varepsilon(x)=0$ inside $B_\varepsilon(x_0)$. Call this extension $\tilde u_\varepsilon$. Notice that this extension lives in $H^1(\Omega)$, since the function values of $\tilde u_\varepsilon$ and both normal and tangential derivative vanish at any point of $\partial B_\varepsilon(x_0)$. Unfortunately, though, these extensions are no longer in $H^2(\Omega)$. Indeed, suppose by contradiction that they were. Consider the difference $\tilde u:= \tilde u_\varepsilon - \tilde u_{\varepsilon/2}$. This function then solves the boundary value problem 
\begin{align*}
\Delta^2 \tilde u (x) &= 0 \ , \ x\in \Omega \ , \\
\tilde u(x) &= \partial_n \tilde u(x) = 0 \ , x\in \partial \Omega \ ,
\end{align*}
which is a contradiction since $\tilde u$ does not vanish. Hence we require a different approach.

\paragraph*{Bounding the $H^2$-norm} We seek to bound the $H^2$-norm of $u_\varepsilon$ independently of $\varepsilon$ in order to apply a compactness argument. Let $\Omega_\varepsilon : = \Omega \setminus B_\varepsilon(x_0)$.

\begin{lemma}
$\int_{\Omega_\varepsilon} |\Delta u_\varepsilon|^2 dx$ is bounded from above independently of $\varepsilon$. 
\end{lemma}
\begin{proof}
%Let $u\in H^2(\Omega)$ be the solution of 
%\begin{align*}
%\Delta^2 u (x) &= 0 \ , \ x\in \Omega \ , \\
%u(x) &=f(x) \ , \ \partial_n u(x) = g(x) \ , x\in \partial \Omega \ . 
%\end{align*}
Integration by parts yields
\begin{align*}
\int_{\Omega_\varepsilon} |\Delta u_\varepsilon|^2 dx 
&= -\int_{\Omega_\varepsilon} \nabla (\Delta u_\varepsilon) \cdot  \nabla (u_\varepsilon)dx + \int_{\partial \Omega_\varepsilon} \Delta u_\varepsilon \partial_n u_\varepsilon ds \\ 
&= -\int_{\Omega_\varepsilon} \nabla (\Delta u_\varepsilon) \cdot  \nabla (u_\varepsilon)dx + \int_{\partial \Omega} \Delta u_\varepsilon g ds \\ 
&= \int_{\Omega_\varepsilon} (\Delta^2 u_\varepsilon) u_\varepsilon dx + \int_{\partial \Omega} \Delta u_\varepsilon g ds - \int_{\partial \Omega} \partial_n (\Delta u_\varepsilon) f ds \\
&=   \int_{\partial \Omega} \Delta u_\varepsilon g ds -  \partial_n (\Delta u_\varepsilon) f ds . 
\end{align*}
Define the space  
\[
H(\Omega_\varepsilon, \Delta):= \{u \in L^2(\Omega_\varepsilon) \ | \ \Delta u  \in L^2(\Omega_\varepsilon)\} \ , 
\]
equipped with the inner product
\[
(u,v)_{H(\Omega_\varepsilon, \Delta)} = (u,v)_{L^2(\Omega_\varepsilon)} + (\Delta u, \Delta v)_{L^2(\Omega_\varepsilon)} \ .
\]
Then a result by Lions-Magenes (see \emph{Non-homogeneous Boundary value Problems and Applications I, Springer-Verlag, New-York, 1972}) states that the trace operators 
\[
\gamma_0 (u) := u_{|\partial \Omega_\varepsilon} \quad \text{and}  \quad \gamma_1 (u) := \partial_n u_{|\partial \Omega_\varepsilon} 
\]
are continuous and onto $H^{-1/2}(\partial \Omega_\varepsilon)$ and $H^{-3/2}(\partial \Omega_\varepsilon)$ from $H(\Omega_\varepsilon, \Delta)$, respectively.
This implies that 
\begin{align*}
\left |  \int_{\partial \Omega} \Delta u_\varepsilon g ds \right | 
&\leq \| \Delta u_\varepsilon\|_{H^{-1/2}(\partial \Omega_\varepsilon)} \| g\|_{H^{1/2}(\partial \Omega)} \\
&\leq C \| \Delta u_\varepsilon\|_{L^2(\Omega_\varepsilon)} \| g\|_{H^{1/2}(\partial \Omega)} 
\end{align*}
and likewise 
\begin{align*}
\left |  \int_{\partial \Omega} \partial_n(\Delta u_\varepsilon) f ds \right | 
&\leq \| \partial_n(\Delta u_\varepsilon)\|_{H^{-3/2}(\partial \Omega_\varepsilon)} \| f\|_{H^{3/2}(\partial \Omega)} \\
&\leq C \| \Delta u_\varepsilon\|_{L^2(\Omega_\varepsilon)} \| f\|_{H^{3/2}(\partial \Omega)}  \ .
\end{align*}
This implies the claim.
\end{proof}

\begin{lemma}
$\int_{\Omega_\varepsilon} |\nabla u_\varepsilon|^2 dx$ is bounded from above independently of $\varepsilon$. 
\end{lemma}
\begin{proof}
Integration by parts yields
\begin{align*}
\int_{\Omega_\varepsilon} |\nabla u_\varepsilon|^2 dx
&= -\int_{\Omega_\varepsilon}\Delta u_\varepsilon u_\varepsilon dx + \int_{\partial \Omega_\varepsilon} u_\varepsilon \partial_n u_\varepsilon ds \\ 
&= -\int_{\Omega_\varepsilon}\Delta u_\varepsilon u_\varepsilon dx + \int_{\partial \Omega} fg  ds  \\
&\leq \frac \delta2  \| \Delta u_\varepsilon\|_{L^2(\Omega_\varepsilon)}^2 +  \frac {1}{2\delta}  \| u_\varepsilon\|_{L^2(\Omega_\varepsilon)}^2 + \int_{\partial \Omega} |fg|  ds \quad \text{(by Young)}\\
&\leq \frac {1}{2\delta}  \| u_\varepsilon\|_{L^2(\Omega_\varepsilon)}^2 + C_1 \quad \text{(by previous Lemma)}\ .
\end{align*}
Notice that $u_\varepsilon$ can be extended trivially to all of $\Omega$ by setting it to zero inside $B_\varepsilon(x_0)$ and that $u_\varepsilon \in H^1(\Omega)$ in this way. Let $v\in H^1(\Omega)$ be any fixed function such that $v=f$ along $\partial \Omega$. Then we get 
\begin{align*}
\frac {1}{2\delta}  \| u_\varepsilon\|_{L^2(\Omega_\varepsilon)}^2 
&\leq \frac {1}{2\delta}  \| v- u_\varepsilon\|_{L^2(\Omega)}^2 + \frac {1}{2\delta}  \| v\|_{L^2(\Omega)}^2 \\
&\leq \frac {C}{2\delta}  \| \nabla v- \nabla u_\varepsilon\|_{L^2(\Omega)}^2 + \frac {1}{2\delta}  \| v\|_{L^2(\Omega)}^2 \quad \text{(by Poincar{\' e})}\\
&\leq \frac {C}{\delta}  \| \nabla u_\varepsilon\|_{L^2(\Omega)}^2 + \frac {C}{\delta}  \| \nabla v \|_{L^2(\Omega)}^2 + \frac {1}{2\delta}  \| v\|_{L^2(\Omega)}^2 \\
&= \frac {C}{\delta}  \| \nabla u_\varepsilon\|_{L^2(\Omega_\varepsilon )}^2 + C_2  \ . 
\end{align*}
Setting $\delta := 2C$ finishes the proof.
\end{proof}

A similar argument as in the previous proof (choosing $v\in H^1(\Omega)$ to be any fixed function such that $v=f$ along $\partial \Omega$) shows:
\begin{lemma}
$\int_{\Omega_\varepsilon} |u_\varepsilon|^2 dx$ is bounded from above independently of $\varepsilon$. 
\end{lemma}

This leads to ur first main result.

\begin{theorem}
$\|u_\varepsilon\|_{H^2(\Omega_\varepsilon)}$ is bounded from above independently of $\varepsilon$.
\end{theorem}
\begin{proof}
The squared $H^2$-norm is given by
\[
\|u_\varepsilon\|^2_{H^2(\Omega_\varepsilon)} = \int_{\Omega_\varepsilon} \|\mathrm{Hess} (u_\varepsilon)\|^2_F dx
+ \int_{\Omega_\varepsilon} |\nabla u_\varepsilon|^2 dx + \int_{\Omega_\varepsilon} |u_\varepsilon|^2 dx \ ,
\]
where $\mathrm{Hess} (u_\varepsilon)$ denotes the Frobenius-norm of the Hessian. By the previous lemmas it suffices to bound this first term
\begin{align*}
\int_{\Omega_\varepsilon} \|\mathrm{Hess} (u_\varepsilon)\|^2_F dx &= 
\int_{\Omega_\varepsilon} \sum_{j,k=1}^2 (\partial_{jk} u_\varepsilon)^2 dx  \\
%&=  \sum_{j,k=1}^2 \int_{\Omega_\varepsilon}  (\partial_j\partial_k u_\varepsilon) (\partial_j\partial_k u_\varepsilon) dx \\
&= \int_{\Omega_\varepsilon}  (\Delta u_\varepsilon)^2 dx + 2 \int_{\Omega_\varepsilon}  (\partial_{12} u_\varepsilon) ^2 - (\partial_{11} u_\varepsilon)(\partial_{22} u_\varepsilon)dx \ .
\end{align*}
By the previous lemmas is therefore suffices to bound the last integral from above. Integration by parts yields
\begin{align*}
 \int_{\Omega_\varepsilon}  (\partial_{12} u_\varepsilon)^2 dx 
 &= - \int_{\Omega_\varepsilon}  (\partial_{121} u_\varepsilon) (\partial_2 u_\varepsilon) dx + \int_{\partial \Omega_\varepsilon}  (\partial_2 u_\varepsilon) (\partial_{12} u_\varepsilon) n_1 ds\\
&= \int_{\Omega_\varepsilon}  (\partial_{11} u_\varepsilon) (\partial_{22} u_\varepsilon) dx + \int_{\partial \Omega}  (\partial_2 u_\varepsilon) (\partial_{12} u_\varepsilon) n_1 ds-\int_{\partial \Omega}  (\partial_2 u_\varepsilon) (\partial_{11} u_\varepsilon) n_2 ds\\
&=\int_{\Omega_\varepsilon}  (\partial_{11} u_\varepsilon) (\partial_{22} u_\varepsilon) dx + \int_{\partial \Omega}  (\partial_2 u_\varepsilon) (\partial_{t} \partial_1 u_\varepsilon)  ds \ ,
\end{align*}
where $\partial_t$ denotes the tangential derivative along the boundary. We therefore have to bound
\[
 \int_{\Omega_\varepsilon}  (\partial_{12} u_\varepsilon) ^2 - (\partial_{11} u_\varepsilon)(\partial_{22} u_\varepsilon)dx =  \int_{\partial \Omega}  (\partial_2 u_\varepsilon) (\partial_{t} \partial_1 u_\varepsilon)  ds
\]
from above. Notice that 
\[
\partial_2 u_\varepsilon = ((\partial_t u_\varepsilon) t + (\partial_n u_\varepsilon) n) \cdot \partial_2 = ((\partial_t f) t + g n) \cdot \partial_2 \ .
\]
Therefore, 
\[
|\partial_2 u_\varepsilon|^2 \leq (\partial_t f)^2 + g^2 \ . 
\]
Likewise,
\[
\partial_t(\partial_1 u_\varepsilon) = \partial_t(((\partial_t u_\varepsilon) t + (\partial_n u_\varepsilon) n) \cdot \partial_1) = \partial_t(((\partial_t f) t + g n) \cdot \partial_1) \ .
\]
Applying the product rule, notice that the last term can be bounded by constants involving the curvature of $\partial\Omega$, up to second tangential derivatives of $f$ and up to first tangential derivatives of $g$. This finishes the proof.
\end{proof}

\paragraph*{The limit as $\varepsilon \to 0$} Our main result is the following.
\begin{theorem}
Let $u_\varepsilon$ be as above. Fix $0<\alpha <1$. Extend each $u_{\varepsilon}$ to all of $\Omega$ by setting it zero on $\Omega \setminus \Omega_\varepsilon$. Then there exists a subsequence $(u_{\varepsilon_n})$ such that 
\[
\lim_{n \to \infty} u_{\varepsilon_n}  = u_0 \quad \text{in $C^{0,\alpha}(\Omega)$}  \ ,
\]
with  $u_0(x_0)=0$, $u_0\in H^2(\Omega\setminus \{x_0\})\cap H^1(\Omega)$ and $\Delta^2 u_u(x)=0$ on $\Omega\setminus \{x_0\}$.
\end{theorem}
\begin{proof}
Fix $\delta >0$. By the Sobolev embedding theorem the embedding
\[
H^2(\Omega_\delta) \subset C^{0,\alpha}(\Omega_\delta) 
\]
is compact for all $0<\alpha<1$. By the previous theorem, $u_\varepsilon$ is bounded in $H^2(\Omega_\delta)$ for all $\varepsilon<\delta$ independently of $\varepsilon$. Therefore, there exists a subsequence $(u_{\varepsilon_n})$ such that 
\[
\lim_{n \to \infty} u_{\varepsilon_n}  = u_\delta \quad \text{weakly in $H^2(\Omega_\delta)$ and strongly in $C^{0,\alpha}(\Omega_\delta)$}\ . 
\]
Since each $u_{\varepsilon_n}$ can be trivially extended to all of $\Omega$ by setting it zero on $\Omega \setminus \Omega_\delta$ and since this extension does not change the H{\" o}lder norm, it follows that 
\[
\lim_{n \to \infty} u_{\varepsilon_n}  = u_\delta \quad \text{strongly in $C^{0,\alpha}(\Omega)$}\ . 
\]
By possibly passing to a subsequence, we can assume that 
\[
\| u_{\varepsilon_n}- u_{\varepsilon_m} \|  \leq \delta \quad \text{in $C^{0,\alpha}(\Omega)$ for all $n, m$}\ . 
\]
Possibly passing again to a subsequence, we can repeat this argument for $\delta/2, \delta/4, \delta/8$, and so forth. Taking the resulting diagonal sequence then  finishes the proof.
\end{proof}


==> points.tex <==
\paragraph{Isolated points}
%
%
A very useful \emph{user interface} to many energy minimization problems are
fixed values at isolated points.
%
For interactive shape deformation, a user may specify the transformation at a
few points, hoping that the energy minimization will propagate these smoothly
to the rest of the shape.
%
For scattered data, the fixed values may represented isolated measurements that
high-order energy minimization should interpolate.
%
Advanced data denoising techniques may employ isolated point constraints to
maintain salient extrema \cite{Weinkauf2010,Guenther:FME:2014}.

Points having zero measure are potentially dubious boundary conditions.
%
For example, for the lower Dirichlet energy $∫_Ω ‖∇u‖² \dA$ an
isolated point constraint is \emph{ill-posed}.
%
Indeed, if we consider the point
as the limit of a shrinking circle of fixed values, then for any finite size
the problem is well posed, but in the limit the solution is not smooth (see
\reffig{point-constraints}).

\begin{figure}
\includegraphics[width=\linewidth]{images/pointconstraints/pointconstraints.pdf}
\caption{This figure shows the energy minimization problem with multiple rows
fixed at the boundary (zero Neumann) and one point constraint in the interior.
Dirichlet is degenerate there (the small figures show convergence to a delta
function), while Laplacian with zero Neumann boundary conditions and Hessian
aren't. \label{fig:point-constraints}}
\end{figure}

We can ask whether a similar issue arises when imposing point constraints on
our higher-order energies.
%
Discrete experimentation in the geometry processing literature suggests that
point constraints are well behaved (see, e.g., \cite{Jacobson:MixedFEM:2010}).
%
We confirm this empirically in our experiments with the  $E_{∆²}$ or $E_{\H²}$
energies.
%
%In our supplemental material, we prove under mild assumptions that point
%constraints for biharmonic problems (emanating from minimization of $E_{∆²}$
%or $E_{\H²}$) may be interpreted as the well-posed solution to the limit of a
%shrinking circle when using Dirichlet and Neumann boundary conditions.
%

%
%\paragraph{Theorem} 
%\alec{Should we state a formal theorem here? If so what?}
%\paragraph{Proof} 
%%
%See \refapp{point-constraints-proof}.



==> scattered.tex <==
% !TEX root = hessian.tex

\subsection{Sparse scattered data interpolation}
\label{sec:scattered}

\begin{figure}
 \centering
  \includegraphics[width=\linewidth]{images/planck/plancks.pdf}
  \caption{
  \alec{This is going in the right direction. It's hard to see the differences
  (hence the arrows) and also hard to tell its a face. The full, closed max
  planck model will be immediately recognized as a ``standard'' test shape.
  What about making really random looking holes and missing data like in the
  Lipman paper? We can pretend this is a ``partial scan'' (keep faces randomly
  weighted according to some angle)}
  Scattered data interpolation over a face-shaped domain.
  The Dirichlet and Neumann boundary conditions are fixed at the outer boundary.
  The Laplacian energy with zero Neumann boundary conditions is very sensitive to the positioning and shape of holes, while the Hessian energy is not, as indicated by red arrows.
   \label{fig:scattereddata}}
\end{figure}

Given measured data values $\{s_i\}$ at arbitrary (scattered and not
coincident) positions $\{\mathbf{p_i}\}$, scattered data
interpolation~\cite{Franke82,FrankeNielson:91} seeks a 
smooth (at least $C^1$) function $u(\mathbf{x})$ fitting the data. A
variational approach to this problem seeks to minimize a smoothness
energy subject to the conditions $u(\mathbf{p}_i) = s_i$.
%
%
%\begin{figure}
% \centering
%  \includegraphics[width=\linewidth]{images/scattereddata/scattereddata.pdf}
%  \caption{Scattered data interpolation over a country-shaped
%    domain. The Laplacian energy subject to zero Neumann boundary
%    conditions flattens the data at the boundary. Arrows \textsf{a}
%    and \textsf{b} point to distortion of isolines due to the shape of
%    the boundary. The Hessian energy over $\R^2$ ignores the geometry
%    of the boundary completely and is sensitive to relative
%    arrangement of data samples. Arrow \textsf{c} points to isolines
%    that flow northwest along an open corridor; arrow \textsf{d}
%    points to an information ``leak' from south to north across the
%    boundary. The Hessian energy subject to its natural boundary
%    conditions and data sample conditions alleviates these
%    distortions, and extrapolates the data as linearly as
%    possible (arrow $\textsf{e}$). \label{fig:scattereddata}}
% %\end{center}
%\end{figure}


Consider data samples gathered in a limited region, where the
boundaries of the sampling domain are dictated by ``outside''
considerations, such as politics, economics, practicality, safety, or
opportunity~(see Figs.~\ref{fig:teaser}, \ref{fig:scattereddata}). In
such as case, the boundaries of the sampling domain do not provide any
meaningful \emph{prior} on the behavior of the smooth
function. 


\begin{figure}
 \centering
  \includegraphics[width=0.5\textwidth]{images/smoothing/cathedral.pdf}
  \caption{
  \alec{Convert to a horizontal figure. It might be cute to render a little
  brick building beneath each. Slightly lower frequency noise might help make
  the problem statement more clear.}
  \(L^1\) smoothing of a function representing the roof of a cathedral. The
  Laplacian with zero Neumann boundary conditions fails at the seams where
  piecewise linear functions meet, while the Hessian reconstructs a piecewise
  linear function that would make a nice roof. \label{fig:cathedral}}
 %\end{center}
\end{figure}



Interpolating the data subject to zero Neumann conditions flattens the
data approaching the boundary, distorting the isolines to be normal to the
boundary, whether in the vicinity of isolated (see
Fig.~\ref{fig:scattereddata}-a) or clustered (see
Fig.~\ref{fig:scattereddata}-b) samples. Since the boundary shape
arises due to ``irrelevant'' considerations, the distortion of
isolines due to the shape of the boundary cannot be justified, as it
might have been for a physical boundary.

We might seek to avoid the distortion by simply ignoring the boundary
altogether, solving over the plane. Unfortunately, this approach too introduces
undesirable distortions arising from the relative arrangement of samples.
Isolines distort the flow along undersampled corridors (see
Fig.~\ref{fig:scattereddata}-c, flowing northwest). Data samples ``leak''
causing isoline bulges that are locally inexplicable (see
Fig.~\ref{fig:scattereddata}-d). 

All of these distortions are alleviated by minimizing $E_{\H²}$
subject to its natural boundary conditions and the data sample
constraints. In doing so, we acknowledge both the given samples
\emph{and} the absence of knowledge at the boundary of the sampling
region. In the absence of samples, this approach extrapolates the data
as linearly as possible (see Fig.~\ref{fig:scattereddata}-e).

% Where \(E_S\) is the user's preferred smoothing energy and \((p_i, s_i)\) are
% the interpolation points where values are prescribed. Depending on the
% properties of the smoothing energy, different behavior can be observed. If the
% boundary of the domain represents a physical border to the data (like liquid
% flow in a pipe), zero Neumann conditions should apply, and the Laplacian with
% zero Neumann boundary conditions should be used. If the domain is just a subset
% of a continuing flat region that can be extended, the Hessian over the whole
% domain should be used. If we don't want to make any particular judgement, and
% just say that the data should vary as little as possible over the boundary, the
% Hessian with natural boundary conditions should be used. \\

% Results can be seen in Figures \ref{fig:teaser} and \ref{fig:scattereddata}. As
% it can be seen in Figure \ref{fig:scattereddata}, the Laplacian flattens the
% data at the boundary. This leads to undesirable results especially when the
% boundary is complicated and the data extends linearly over it, as in the
% southern tips of the domain. The Hessian over the whole domain has a different
% problem: it glues together the two southern tips that are separated by a
% valley, even though that assumption might not be justified.



% \alec{belongs in scattered}
% %
% Then the data is assumed to vary only tangential along the boundary: hence the
% boundary's shape will have a strong impact on the solution (see the Fjord's in
% \reffig{teaser}).
% %
% If the boundary of $Ω$ is ignored and $E_\text{smooth}$ is instead defined over 
% a larger Euclidean domain containing $Ω$, then information in the data term $f$
% will \emph{leak} across the $Ω$ (see the ``infinite ocean'' in
% \reffig{teaser}).


==> subspace.tex <==
\subsection{Subspace design}
\label{sec:subspace-design}

Wang et al.~\shortcite{Wang2015} show that subspaces for smooth shape
deformation can be designed using a variational principle when linear functions
exist in the null space of the invoked smoothness energy $E_\text{smooth}$.
Subspace functions (a.k.a, weights) corresponding to the $m$ user-controlled
``handles'' result from energy minimization:
%
\begin{align}
 \argmin_{w_i} E_\text{smooth}(w_i) && \forall i ∈ \{1,\dots,m\} \\
 \text{subject to } w_i(\p_j) = \delta_{ij}    && \forall i,j ∈\{1,\dots,m\},
\end{align}
where $\p_j$ is the location of the $j$th handle and $\delta_{ij}$ is
Kronecker's Delta function. Deformations of a point $\p$ on the domain is then
simply the weighted combination of handle positions: $\p → ∑_{i=1}^m w_i(\p)
\p_i$.
%
In \cite{Wang2015}, the discrete smoothness energy $E_\text{smooth}→E_{W}$is a
modified form of $E_{∆²}$ (see discussion in \refsec{lsd}). 


The squared Hessian energy $E_{\H²}$ has \emph{exactly} linear functions in its
null space. 
%
This structure is preserved by our finite difference discretization.
%
This makes $E_{\H²}$ immediately useful for defining subspace deformation
weights.

Experimental evidence suggests that weights computed using $E_{\H²}$ are much
more stable with respect to shape boundary and handle locations than $E_W$ (see
\reffig{crosses}).
%
This has important ramifications for subspace deformation.
%
As originally observed in \cite{Wang2015}, a small change in handle locations
can dramatically affect the solution (see \reffig{checkerboard}). In contrast,
the subspace built with $E_{\H²}$ is stable: a small change to the handles
results in a small change in the deformation.

Wang et al. propose the concept of ``extra handles'', controlled not directly
by the user but instead by minimizing a non-linear deformation energy (e.g.,
the as-rigid-as-possible energy) in the weight-based subspace
\cite{Jacobson:FAST:2012}.
%
With a small number of extra handles, the stability issues with $E_W$ persist.
%
Figure \ref{fig:giraffe} shows that both methods perform similarly with a large
number of 
extra handles controlled via the same as-rigid-as-possible optimization.
%
However, when the number of extra handles is reduced (and the subspace made
more efficient), the $E_{\H²}$ weights degrade gracefully, while $E_W$'s
instabilities quickly appear. 

Our subspace makes it easier to create pleasing-looking animations,as seen in
Figure \ref{fig:cheeseman}.
%
Smaller changes in in the user's constraints do not lead to visually jarring
changes.

